RASA: Efficient Register-Aware Systolic Array Matrix Engine for CPU

As AI-based applications become pervasive, CPU vendors are starting to incorporate matrix engines within the datapath to boost efficiency. Systolic arrays have been the premier architectural choice as matrix engines in offload accelerators. However, we demonstrate that incorporating them inside CPUs can introduce under-utilization and stalls due to limited register storage to amortize the fill and drain times of the array. To address this, we propose RASA, Register-Aware Systolic Array. We develop techniques to divide an execution stage into several sub-stages and overlap instructions to hide overheads and run them concurrently. RASA-based designs improve performance significantly with negligible area and power overhead.

==> algorithms/convolution.tex <==
\begin{algorithm}[t]
% \scriptsize
%\footnotesize
\SetInd{0.45em}{0.45em}
\SetAlgoLined
\DontPrintSemicolon
\KwIn{ \TODO{Fix here} \\
\textit{IA}: input\_activation [n][c][x][y] \\
\textit{OA}: output\_activation [k][c][x][y] \\
\textit{F}: The array of filters [k][c][r][s] \\
\textit{stride}: stride\\

\\
}
%dataflow\_candidates $\leftarrow$ {\scriptsize \textbf{get\_candidate\_LoopOrders\_ClusterSzs}(\textit{Arch}, \textit{P})};\\
%\textit{num\_LoopOrders} $\leftarrow$ {\scriptsize \textbf{get\_num\_LoopOrders}(dataflow\_candidates)};\\ \textit{num\_ClusterSzs} $\leftarrow$ {\scriptsize \textbf{get\_num\_ClusterSzs}(dataflow\_candidates)};\\

% \textit{num\_LoopOrders} $\leftarrow$ dataflow\_candidates.shape[0]; \textit{num\_ClusterSzs} $\leftarrow$ dataflow\_candidates.shape[1];\\

% \Comment*[r]{\textbf{\textcolor{blue}{num\_LoopOrders = candidate\_dataflows.shape[0]}}}
% \Comment*[r]{\textbf{\textcolor{blue}{num\_ClusterSzs = candidate\_dataflows.shape[1]}}}

\For{n $=$ 0 \KwTo N-1}{
    \For{k $=$ 0 \KwTo K-1}{
        \For{x $=$ 0 \KwTo (X-R) / stride}{
            \For{y $=$ 0 \KwTo (Y-S) / stride}{
                \For{c $=$ 0 \KwTo C-1}{
                    \For{r $=$ 0 \KwTo R-1}{
                        \For{s $=$ 0 \KwTo S-1}{
                            xx = x*stride + r \\
                            yy = y*stride + s \\
                            OA[n][k][x][y] = IA[n][k][xx][yy] * F[k][c][r][s]
        
                        }
                    }
                }
            }
        }
    }
}

\caption{Convolution Operation in CNN}
\label{alg:flash_setup}
\end{algorithm}

==> algorithms/gemm.tex <==
\begin{algorithm}[t]
% \scriptsize
%\footnotesize
\SetInd{0.45em}{0.45em}
\SetAlgoLined
\DontPrintSemicolon
\KwIn{ \TODO{Fix here} \\
M = N = K = 32, GEMM with BF16 and FP 32 for input and output data types.
\\
}
%dataflow\_candidates $\leftarrow$ {\scriptsize \textbf{get\_candidate\_LoopOrders\_ClusterSzs}(\textit{Arch}, \textit{P})};\\
%\textit{num\_LoopOrders} $\leftarrow$ {\scriptsize \textbf{get\_num\_LoopOrders}(dataflow\_candidates)};\\ \textit{num\_ClusterSzs} $\leftarrow$ {\scriptsize \textbf{get\_num\_ClusterSzs}(dataflow\_candidates)};\\

% \textit{num\_LoopOrders} $\leftarrow$ dataflow\_candidates.shape[0]; \textit{num\_ClusterSzs} $\leftarrow$ dataflow\_candidates.shape[1];\\

% \Comment*[r]{\textbf{\textcolor{blue}{num\_LoopOrders = candidate\_dataflows.shape[0]}}}
% \Comment*[r]{\textbf{\textcolor{blue}{num\_ClusterSzs = candidate\_dataflows.shape[1]}}}
\vspace{5}

// load C Tiles to tmm registers \\
%tileloadd tmm0, ptr [rax+r11*4] \\
\textit{tileloadd} tmm0, ptr[CTile0]  \\
\textit{tileloadd} tmm1, ptr[CTile1] \\
\textit{tileloadd} tmm2, ptr[CTile2] \\
\textit{tileloadd} tmm3, ptr[CTile3] \\
\texttt{\\}
// Compute partial sums\\
\textit{tileloadd} tmm4 BTile0 \\
\textit{tileloadd} tmm6 ATile0 \\
\textit{tdpbf16ps} tmm0, tmm6, tmm4 \\
\textit{tileloadd} tmm5 BTile1 \\
\textit{tdpbf16ps} tmm2, tmm6, tmm5 \\
\textit{tileloadd} tmm7 ATile1 \\
\textit{tdpbf16ps} tmm1, tmm7, tmm4 \\
\textit{tdpbf16ps} tmm3, tmm7, tmm5 \\
\texttt{\\}
// store C Tiles to tmm registers \\
\textit{tilestored} ptr[CTile0], tmm0 \\ 
\textit{tilestored} ptr[CTile1], tmm1 \\
\textit{tilestored} ptr[CTile2], tmm2 \\
\textit{tilestored} ptr[CTile3], tmm3 \\

%tilestored ptr [r12+r14*4], tmm0


\caption{GEMM Example with AMX instructions}
\label{alg:flash_setup}
\end{algorithm}

==> sections/7_acknowledgements.tex <==
\section*{Acknowledgment}
Put sponsor acknowledgments in the unnumbered footnote on the first page.

Capitalize only the first word in a paper title, except for proper nouns and element symbols.
